"I understand why I got this grade": Automatic Short Answer Grading with Feedback

In recent years, there has been a growing interest in using Artificial Intelligence (AI) to automate student assessment in education. Among different types of assessments, summative assessments play a crucial role in evaluating a student's understanding level of a course. Such examinations often involve short-answer questions. However, grading these responses and providing meaningful feedback manually at scale is both time-consuming and labor-intensive. Feedback is particularly important, as it helps students recognize their strengths and areas for improvement. Despite the importance of this task, there is a significant lack of publicly available datasets that support automatic short-answer grading with feedback generation. To address this gap, we introduce Engineering Short Answer Feedback (EngSAF), a dataset designed for automatic short-answer grading with feedback. The dataset covers a diverse range of subjects, questions, and answer patterns from multiple engineering domains and contains ~5.8k data points. We incorporate feedback into our dataset by leveraging the generative capabilities of state-of-the-art large language models (LLMs) using our Label-Aware Synthetic Feedback Generation (LASFG) strategy. This paper underscores the importance of enhanced feedback in practical educational settings, outlines dataset annotation and feedback generation processes, conducts a thorough EngSAF analysis, and provides different LLMs-based zero-shot and finetuned baselines for future comparison. The best-performing model (Mistral-7B) achieves an overall accuracy of 75.4% and 58.7% on unseen answers and unseen question test sets, respectively. Additionally, we demonstrate the efficiency and effectiveness of our ASAG system through its deployment in a real-world end-semester exam at a reputed institute.

==> neurips_data_2023/sections/RelevanceToTheSociety.tex <==
\section{Relevance to the society}

In today's rapidly evolving educational landscape, assessing and evaluating student's learning outcomes play a vital role in shaping the quality of education. Digital technology has ushered in transformative changes, and one such advancement is the development of ASAG systems. This section discusses the relevance of our research on ASAG to the broader society and education system.
\subsection{Enhancing Efficiency and Accessibility}

 Due to very high student-to-teacher ratio in the educational field,  traditional manual grading methods frequently consume a significant amount of educator's time, limiting their ability to provide students with timely and constructive feedback. To support this argument, reference to \textbf{2011} data reveals that in the realm of secondary education, \textbf{India} exhibits a students per teacher ratio of \textbf{25.92}. In contrast, for countries like \textbf{Central African Republic (CAR)} and \textbf{Croatia}, the corresponding students per teacher ratios are \textbf{66.82} and \textbf{8}, respectively.
    Given the varying student-to-teacher ratios within India and around the world, which can be seen from Table \ref{fig:student_teacher_ratio}, there arises a critical need for innovative solutions to manage assessment and feedback processes effectively. In this section, data values have been taken from nationmaster website  \footnote{\url{https://www.nationmaster.com/country-info/stats/Education/Pupil--teacher-ratio,-secondary#2011}}. Here's how improving ASAG systems can address these challenges:
\begin{itemize}
    
    \item \textbf{Scalability}: In countries like \textbf{Central African republic (CAR)}, \textbf{Malawi} with relatively high student-to-teacher ratios, automating the grading process becomes crucial. An ASAG system can efficiently handle a large volume of student responses.
    \item \textbf{Timely Feedback}: With larger class sizes, providing timely and constructive feedback to each student becomes challenging. An automated grading system can offer immediate feedback.
    \item \textbf{Standardization}: Automated grading ensures a consistent and objective evaluation process. This is especially important in cases where differences in educator expertise or subjectivity may result in uneven grading standards.
\end{itemize}




\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{Images/student_teacher_ratio (3).png}
    \caption{2011 Student-teacher ratio for secondary education among different countries in the world.}
    \label{fig:student_teacher_ratio}
\end{figure*}


% \begin{figure} % Use figure* for spanning across two columns
%   \centering % Center the figure
%   \includegraphics[width=0.5\textwidth]{AnonymousSubmission/Images/student_teacher_ratio.png} % Include your image with desired width
%   \caption{ Frequency Chart of Labels in the Dataset} % Add your caption here
%   \label{fig:labels_distribution} % Add a label for referencing
% \end{figure}

% \subsection{Enhancing Efficiency and Accessibility}
% In \textbf{India}, for primary school the latest value from 2017 is \textbf{32.75} students per teacher. For comparison, the world average in 2017 based on \textbf{132 countries} is \textbf{21.75} students per teacher.\footnote{https://www.theglobaleconomy.com/India/student\_teacher\_ratio
%     \_primary\_school} Due to this high student-to-teacher ratio,  traditional manual grading methods frequently consume a significant amount of educators' time, limiting their ability to provide students with timely and constructive feedback. Our research aims to streamline the assessment process by leveraging the power of automated grading systems.

==> neurips_data_2023/sections/background.tex <==
\section{Background and Definitions}
\begin{itemize}
    \item \textbf{AI-assisted short answer grading: }AI-assisted short answer grading refers to the use of Artificial Intelligence algorithms to grade short answer assessments. These algorithms analyze student answers and assign a real-valued score based on the accuracy, completeness, and relevance of the answers. AI-assisted grading can provide objective and consistent grading, reducing the possibility of human error and subjectivity. Additionally, AI-assisted grading can save time and effort compared to manual grading, allowing instructors and teachers to focus on more important tasks such as providing feedback and engaging with students.

\end{itemize}


==> neurips_data_2023/sections/modeling.tex <==
% \section{Modeling}


\section{Block Diagram and Model Architecture}
\label{architecture}

This section presents the architectural frameworks employed in our study for ASAG. We investigate two distinct architectures, each tailored to address the grading of short answers.

\subsection{Pretrained Language Models (PLMs) for sequence classification}
We use different BERT \cite{devlin2018bert} based models for sequence classification, and we further subdivide this architecture into two categories based on the input passed to the model as shown in figure \ref{fig:bertForClassification}.
\begin{enumerate}
    \item \textbf{Without Question}: Student answer and Reference answer are passed as input to the model as shown in figure \ref{fig:a}.
    \item \textbf{With Question}: Question, Student answer, and Reference answer are passed as input to the model as shown in figure \ref{fig:b}.
\end{enumerate}

\subsection{Sentence Transformer models for classification}
We use a pre-trained sentence transformer model and fine-tune it for the task of ASAG. The student answer and reference answer corresponding to a particular question are passed as input to the sentence transformer model and a softmax classifier is applied on top of it to assign each student answer an output label as shown in Figure \ref{fig:sentence-transformer}.
% We have used SBERT and fine-tuned it for the task of ASAG. We have taken the desired answer and the student's answer corresponding to a particular question as input to the SBERT model and by using the CLS token embedding, which contains the representation of the input we have trained a classification neural network for predicting the marks for the particular student response. In Figure ???????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{fig:Bert-architecture} we can see how the desired answer and student answer are passed as input to the BERT model.



% \begin{figure*}
% \centering
%  \includegraphics[width=\linewidth]{block.png}
% \caption{Basic Encoder-Decoder Architecture}
% \label{fig:1}
% \end{figure*}
% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{block.png}
% \caption{fig 1}
% \label{figure1}
% \end{figure}



\begin{figure*}
     \centering
     % \begin{subfigure}[b]{0.3\textwidth}
     %     \centering
     %     \includegraphics[width=\textwidth]{Images/Sentence_tranformer_without_question (1).pdf}
     %     \caption{y=xy=x}
     %     \label{fig:y equals x}
     % \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Images/BERT without question classification.pdf}
         \caption{For the task of ASAG, both the Student answer and the Reference answer separated by the [SEP] token is  passed as input to the BERT model.}
         \label{fig:a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Images/BERT with question classification.pdf}
         \caption{For the task of ASAG, The Question, Student answer, and the Reference answer separated by the [SEP] token is passed as input to the BERT model.}
         \label{fig:b}
     \end{subfigure}
     \hfill
     \caption{Figure (a) and (b) differ on the input passed to the BERT model. In Figure (a) The Student and Reference answer is passed as input while in Figure (b) The Question is also passed alongside the Student and Reference answer as input to the model. The model's output, represented by the CLS embedding, was then processed through a softmax classifier to derive a label for each student answer denoting its level of correctness against the reference answer.}
     \label{fig:bertForClassification}
\end{figure*}



\begin{figure}[t] % Use figure* for spanning across two columns
  \centering % Center the figure
  \includegraphics[width=0.50\textwidth]{Images/Sentence_tranformer_without_question (1).pdf} % Include your image with desired width
  \caption{A Sentence Transformer model, fine-tuning for the ASAG task, takes both the student and reference answers as input. The model processes these answers to produce embeddings, denoted as `u' and `v,' and subsequently concatenates them with their absolute element-wise difference $|u-v|$. The resulting representation is then passed through the topmost Softmax classifier layer, which classifies each student's answer into one of three distinct labels: `correct,' `partially correct,' or `incorrect.'} % Add your caption here
  \label{fig:sentence-transformer} % Add a label for referencing
\end{figure}




